Direct Regret Optimization in Bayesian Optimization

Bayesian optimization (BO) is a powerful paradigm for optimizing expensive black-box functions. Traditional BO methods typically rely on separate hand-crafted acquisition functions and surrogate models for the underlying function, and often operate in a myopic manner. In this paper, we propose a novel direct regret optimization approach that jointly learns the optimal model and non-myopic acquisition by distilling from a set of candidate models and acquisitions, and explicitly targets minimizing the multi-step regret. Our framework leverages an ensemble of Gaussian Processes (GPs) with varying hyperparameters to generate simulated BO trajectories, each guided by an acquisition function drawn from a pool of conventional choices and terminated by a Bayesian early stop criterion. These trajectories train an end-to-end Decision Transformer that selects the next query so as to improve the ultimate objective, following a dense training sparse learning paradigm: the transformer is trained on abundant simulated data, while a limited number of real evaluations refine the GPs online. On synthetic and real-world benchmarks, our method attains the best or near-best final simple regret against standard, lookahead, trust-region and amortized BO baselines, with the largest gains in high-dimensional settings. Ablations attribute the gains jointly to region-of-interest filtering and the learned policy, and matched-budget comparisons against explicit two-step lookahead acquisitions show that the advantage is not shared by lookahead alone.

==> T0-Outline.tex <==
\begin{abstract}
In this article, we propose a unified framework to directly optimize the regret in Bayesian Optimization. 
We draw insights from recent advances in end-to-end model learning, multi-step acquisition optimization, 
and reinforcement learning to deliver an approach that is both theoretically grounded and empirically robust. 
We illustrate how the framework can be applied to various application scenarios (e.g.\ high-dimensional, 
multi-objective, cost-aware optimization) and provide analyses of its performance guarantees.
\end{abstract}

\section{Motivation}
\begin{enumerate}[label=\arabic*]
    \item \textbf{Recent development in end-to-end model learning and acquisition optimization shows advantage over conventional two-stage bi-level optimization.}
    \begin{itemize}
        \item Traditional Bayesian Optimization (BO) techniques often involve sequentially optimizing acquisition functions in a two-stage process.
        \item End-to-end approaches aim to optimize model and acquisition jointly, which can yield improved performance.
    \end{itemize}

    \item \textbf{Generalize the idea to direct regret optimization.}
    \begin{itemize}
        \item Instead of indirectly optimizing regret through acquisition functions, we propose a framework that targets regret directly.
        \item This direct approach may offer more transparent performance bounds and improved convergence properties.
    \end{itemize}

    \item \textbf{Previous works explored RL in BO; we further improve the non-myopic from two perspectives.}
    \begin{enumerate}[label=\roman*)]
        \item Use Gaussian Process (GP) + Acquisition Functions as a warm-start / simulator for policy learning.
        \item Simplify the state space with theoretical insights.
    \end{enumerate}

    \item \textbf{We further incorporate insights into the uncertainty reduction in conventional GP to adjust policy randomness accordingly.}
    \begin{itemize}
        \item Balancing exploration and exploitation is a core concept in Bayesian Optimization.
        \item Our method modulates policy randomness in line with posterior uncertainty, enhancing sampling efficiency.
    \end{itemize}
\end{enumerate}

\section{Thoughts}
\begin{enumerate}[label=\arabic*)]
    \item \textbf{Efficient non-myopic}
    \begin{enumerate}[label=\alph*)]
        \item Well-defined space and action
        \begin{itemize}
            \item \textit{States:} Kernel hyperparameters + Region-of-Interest (ROI) characteristics.
            \item \textit{Action:} Next single or batched query.
        \end{itemize}
    \end{enumerate}

    \item \textbf{Offline training for RL policy --- differentiate from conventional RL / BO}
    \begin{enumerate}[label=\alph*)]
        \item \textit{General vision:}
        \begin{itemize}
            \item Dense training, Sparse Learning: For a GP with several hyperparameters, use it as a simulator to train a decision-making model (e.g.\ transformer) that maximizes ultimate candidate optimality.
        \end{itemize}
        \item \textit{With-model sample:}
        \begin{itemize}
            \item Utilize GP-based samples to guide RL policy updates.
        \end{itemize}
    \end{enumerate}

    \item \textbf{Efficient RL}
    \begin{enumerate}[label=\alph*)]
        \item Warm-start with a few-shot conventional BO.
        \item Early stopping to limit computational overhead.
        \item Transformer as policy network.
        \item Bootstrapping or other caching methods for training efficiency.
    \end{enumerate}

    \item \textbf{Approximation aware}
    \begin{itemize}
        \item By directly optimizing the regret, we can decouple an upper bound of it into model fitness error and true regret.
        \item This helps in understanding and controlling the sources of approximation error.
        \item We use a spectrum of GPs for offline training. This marginalize out the parameter of the GP.
    \end{itemize}

    \item \textbf{Uncertainty is intrinsic in BO and in the policy}
    \begin{itemize}
        \item Without incorporating uncertainty, the model might be confused in the early stage of BO.
        \item Initial exploration is crucial; sub-modularity guarantees the posterior convergence.
        \item We propose reducing randomness in the policy over time, possibly via a learned schedule rather than a fixed temperature parameter.
    \end{itemize}
\end{enumerate}

\section{Objective}
\begin{enumerate}[label=\arabic*)]
    \item \textbf{A unified framework for:}
    \begin{itemize}
        \item Batched optimization.
        \item High-dimensional optimization (especially for ESM-based BO).
        \item Multi-objective optimization.
        \item Cost-aware optimization.
        \item Level-set estimation.
        \item Multi-fidelity optimization.
    \end{itemize}

    \item \textbf{Theoretically sound}
    \begin{itemize}
        \item Guarantee \emph{Positive Definite and Stationary (PDS)} kernel properties.
        \item Mimic neural bandit analysis on top of NTK (Neural Tangent Kernel) convergence guarantees.
        \item Guarantee sub-modularity of the selection process.
        \item Ultimately, guarantee regret bounds.
    \end{itemize}

    \item \textbf{Comprehensive empirical results}
    \begin{itemize}
        \item Comparative studies with conventional BO baselines.
        \item Ablation studies on kernel hyperparameters, model architectures, etc.
        \item Real-world benchmarks in high-dimensional search, multi-objective scenarios, and more.
    \end{itemize}
\end{enumerate}




==> T4-method-brief.tex <==
\section{Method}
\label{sec:method}

In this section, we introduce our Direct Regret Optimization (DRO) approach. DRO departs from conventional Bayesian Optimization (BO) methods by directly targeting the minimization of final optimization regret. The core strategy simulates diverse BO trajectories using an ensemble of Gaussian Process (GP) models. These simulations, constrained within an adaptively identified Region of Interest (ROI), train a decision transformer to propose candidate points predicted to yield the lowest simple regret at the BO horizon.

\subsection{Ensemble of Gaussian Processes and ROI Filtering}
\label{subsec:ensemble_roi}
At each BO step $t$, DRO maintains an ensemble of $M$ GP surrogate models, $\{ \mathrm{GP}_1, \ldots, \mathrm{GP}_M \}$, each with distinct, potentially adapted, hyperparameters and conditioned on the historical data $\mathcal{D}_{t-1} = \{ (\mathbf{x}_i, y_i)\}_{i=1}^{t-1}$. This captures diverse beliefs about $f$.
To focus simulations, an adaptive Region of Interest (ROI) $\hat{\mathcal{X}}_t \subseteq \mathcal{X}$ is identified, akin to BALLET \cite{Zhang2023ROI}. This uses a global-view GP (e.g., an ensemble member or separate model on $\mathcal{D}_{t-1}$) to compute its posterior mean $\mu_{global,t-1}(\mathbf{x})$ and standard deviation $\sigma_{global,t-1}(\mathbf{x})$. The ROI is then defined as:
\begin{equation}
    \hat{\mathcal{X}}_t = \{ \mathbf{x} \in \mathcal{X} \mid \mu_{global,t-1}(\mathbf{x}) + \beta_t^{1/2}\sigma_{global,t-1}(\mathbf{x}) \ge \max_{\mathbf{x}' \in \mathcal{X}} (\mu_{global,t-1}(\mathbf{x}') - \beta_t^{1/2}\sigma_{global,t-1}(\mathbf{x}')) \}.
    \label{eq:roi_definition_condensed}
\end{equation}
This ROI $\hat{\mathcal{X}}_t$ constrains subsequent rollout simulations to promising regions.

\subsection{Simulated Rollouts and Decision Transformer Training}
\label{subsec:rollouts_dt}
For each $\mathrm{GP}_m$ in the ensemble, multiple rollout trajectories are generated. In each simulation step $\tau$, a point $\mathbf{x}_\tau^{(m)} = \underset{\mathbf{x}\in\hat{\mathcal{X}}_t}{\operatorname{argmax}} \; \alpha\bigl(\mathbf{x}; \mathrm{GP}_m, \mathcal{D}_{t-1}^{(\tau, m)}\bigr)$ is selected within $\hat{\mathcal{X}}_t$ using a conventional acquisition function $\alpha$ (e.g., EI, UCB) based on $\mathrm{GP}_m$'s current state. The objective $f(\mathbf{x}_\tau^{(m)})$ is simulated by sampling from $\mathrm{GP}_m$'s predictive distribution. Rollouts terminate via a Bayesian early stop (BES) if the expected improvement within $\hat{\mathcal{X}}_t$ drops below a threshold $\delta$: $\mathbb{E}_{p_m}[\max(0, f(\mathbf{x}_{\text{next}}) - f(\mathbf{x}_{\text{best\_sim}}))] < \delta$. This yields diverse, variable-length simulated trajectories. An ensemble of acquisition functions can further diversify these rollouts.

These trajectories form an offline dataset for training a decision transformer \cite{chen2021decision}. Each trajectory is processed into (state, action, return-to-go) sequences: \textbf{State ($\mathbf{s}_\tau$)} embeds BO progress (GP features, simulation history); \textbf{Action ($\mathbf{a}_\tau$)} is the simulated $\mathbf{x}_\tau^{(m)}$; and \textbf{Return-to-Go ($R_\tau$)} reflects the trajectory's final simple regret. The transformer is trained to predict actions leading to low regret. During real BO, this trained transformer, conditioned on the current real BO state and a high target return (low regret), proposes the next candidate point $\mathbf{x}_t$.

\subsection{Overall DRO Procedure and Learning Paradigm}
The iterative DRO procedure (Algorithm~\ref{alg:direct-regret-optimization}) at each time step $t$ involves: (1) Updating the GP ensemble and $\mathrm{GP}_{global}$ with $\mathcal{D}_{t-1}$. (2) Identifying the ROI $\hat{\mathcal{X}}_t$. (3) Generating simulated rollouts within $\hat{\mathcal{X}}_t$ for each $\mathrm{GP}_m$. (4) Aggregating these trajectories to train/fine-tune the decision transformer. (5) Using the transformer to propose $\mathbf{x}_t$. (6) Evaluating $f(\mathbf{x}_t)$ to get $y_t$ and augmenting $\mathcal{D}_t$. The training objective for the decision transformer is the minimization of the final simple regret $R_{T_{real}} = f^* - f(\mathbf{x}_{T_{real}}^+)$, by leveraging diverse, multi-step simulated trajectories.

% \todo{multi-output transformer to accommodate multi-objective, multi-fidelity, constrained setting.}
% \todo{can we replace transformer with functional GP?}
% \todo{equivalent to BALLET + RL}
% \todo{theoretical solution to the expected reward at $T$?}

\begin{algorithm}[t]
\caption{Direct Regret Optimization with ROI Filtering}
\label{alg:direct-regret-optimization}
\begin{algorithmic}[1]
    \REQUIRE Initial dataset $\mathcal{D}_0$, ensemble size $M$, max real iterations $T_{real}$, early stop threshold $\delta$, num\_rollouts\_per\_gp $K$, ROI parameters (e.g., $\beta_t$)
    \FOR{$t = 1$ to $T_{real}$}
        \STATE \textbf{Fit/Update GPs}: Update $\mathrm{GP}_m$ for $m=1 \dots M$ (and $\mathrm{GP}_{global}$ if separate) using $\mathcal{D}_{t-1}$.
        \STATE \textbf{Identify ROI}: Determine $\hat{\mathcal{X}}_t \leftarrow \{ \mathbf{x} \in \mathcal{X} \mid \mathrm{UCB}_{global,t}(\mathbf{x}) \ge \max_{\mathbf{x}' \in \mathcal{X}} \mathrm{LCB}_{global,t}(\mathbf{x}') \}$ using $\mathrm{GP}_{global}$.
        \STATE \textbf{Initialize} simulation buffer $\mathcal{B}_{sim} \gets \{\}$.
        \FOR{$m = 1$ to $M$}
            \FOR{$k = 1$ to $K$}
                \STATE Simulate rollout $\mathcal{T}_{m,k} = \{(\mathbf{s}_\tau, \mathbf{a}_\tau, R_\tau)\}_{\tau=0}^{L_{m,k}-1}$ using $\mathrm{GP}_m$, acq. $\alpha$ over $\hat{\mathcal{X}}_t$, and BES.
                \STATE Add $\mathcal{T}_{m,k}$ to $\mathcal{B}_{sim}$.
            \ENDFOR
        \ENDFOR
        \STATE \textbf{Train/Update Decision Transformer} on $\mathcal{B}_{sim}$ to minimize final regret.
        \STATE \textbf{Infer Next Candidate} $\mathbf{x}_t \gets \mathrm{DecisionTransformer}(\text{current real state } \mathbf{s}_t, \text{target return } R_{\text{target}})$.
        \STATE Evaluate $y_t = f(\mathbf{x}_t)$ and augment real data $\mathcal{D}_t \gets \mathcal{D}_{t-1} \cup \{(\mathbf{x}_t, y_t)\}$.
    \ENDFOR
\end{algorithmic}
\end{algorithm}

DRO employs a \textbf{dense training--sparse learning} paradigm. \textit{Dense training} occurs as the decision transformer learns non-myopic policies from a large corpus of simulated trajectories generated offline (within each BO step) by the GP ensemble within the ROI. This provides rich supervisory signals on multi-step outcomes. \textit{Sparse learning} happens with each costly real function evaluation $f(\mathbf{x}_t)$, which updates the GP ensemble and grounds the system in the true objective, refining the ROI and potentially the transformer. This dual approach, augmented by ROI filtering, aims for sample-efficient learning of policies robust to model misspecification by leveraging inexpensive, focused simulations for exploration and costly real evaluations for grounding and exploitation.

\subsection{Theoretical Analysis}
The theoretical underpinnings of DRO present a rich area for future investigation. We aim to provide insights into key mechanisms like ROI filtering and the behavior of metrics like Expected Improvement (EI) when regret converges. Formal statements are deferred to Appendix~\ref{sec:theory}. % Replace sec:theory with your actual appendix label if different
% \todo{add skeleton to analyze BO performance when assuming that the model distill a policy that directly optimize the end-of-time expected regret through combination of off-policy learning on the optimization trajectories and on-policy learning by the ensemble of GPs. Here the samples construct the MC estimation over a spectrum of GPs and acquisitions on the ultimate expected regret. }

\paragraph{Regret Guarantees with ROI-Constrained Base Acquisition.}
Constraining a base acquisition function with known cumulative regret guarantees to the adaptively identified ROI (Equation~\ref{eq:roi_definition_condensed}, akin to \cite{Zhang2023ROI}) is expected to largely preserve these guarantees. Performance should then scale with ROI characteristics, incurring a minor penalty for the small probability ($ \sum \delta_t $) of the optimum falling outside this focused region (see Appendix~\ref{sec:theory}).

\paragraph{Convergence of Expected Improvement with Converging Simple Regret.}
If a BO algorithm effectively minimizes simple regret to zero (w.h.p.), the maximum Expected Improvement (EI) across the search space should also converge to zero. As the known optimum is approached, the potential for further gain diminishes, a behavior EI should reflect under a consistent GP model. This is relevant for justifying EI-based early stopping in simulations (see Appendix~\ref{sec:theory}).

==> T8-checklist.tex <==
\section*{Checklist}

\begin{enumerate}

  \item For all models and algorithms presented, check if you include:
  \begin{enumerate}
    \item A clear description of the mathematical setting, assumptions, algorithm, and/or model. [Yes] The setting is formalized in \secref{sec:problem-formulation}, the algorithm in \secref{sec:method} and \algoref{alg:direct-regret-optimization}, and the assumptions of the theoretical results in \appref{sec:theory}.
    \item An analysis of the properties and complexity (time, space, sample size) of any algorithm. [Yes] Computational complexity is discussed at the end of \secref{sec:method}; wall-clock measurements are in \appref{subsec:time}.
    \item (Optional) Anonymized source code, with specification of all dependencies, including external libraries. [Yes] Provided as supplementary material, with pinned dependencies and run configurations.
  \end{enumerate}

  \item For any theoretical claim, check if you include:
  \begin{enumerate}
    \item Statements of the full set of assumptions of all theoretical results. [Yes] Each result in \appref{sec:theory} states its assumptions explicitly.
    \item Complete proofs of all theoretical results. [Yes] Complete proofs are given in \appref{sec:theory} for all results except Lemmas~\ref{lem:infogain} and~\ref{lem:lengthscale}, which are quoted from prior work with citations to the specific results.
    \item Clear explanations of any assumptions. [Yes] Each assumption in \appref{sec:theory} is accompanied by a discussion of when it holds and how it relates to the algorithm.
  \end{enumerate}

  \item For all figures and tables that present empirical results, check if you include:
  \begin{enumerate}
    \item The code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL). [Yes] Provided in the supplementary material.
    \item All the training details (e.g., data splits, hyperparameters, how they were chosen). [Yes] \secref{sec:setup}, \appref{sec:implementation_details} and the configuration files in the supplementary material.
    \item A clear definition of the specific measure or statistics and error bars (e.g., with respect to the random seed after running experiments multiple times). [Yes] \secref{sec:setup}: best observed objective or simple regret, mean $\pm$ one standard error over at least 10 seeded trials; paired tests are reported where used (\appref{sec:additional_results}).
    \item A description of the computing infrastructure used. (e.g., type of GPUs, internal cluster, or cloud provider). [Yes] \appref{subsec:time} (Apple-silicon laptop CPU and a shared 96-core AMD server; no GPUs).
  \end{enumerate}

  \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets, check if you include:
  \begin{enumerate}
    \item Citations of the creator If your work uses existing assets. [Yes] BoTorch, PFNs4BO, SCoreBO, TuRBO, YAHPO Gym, Bayesmark and Gymnasium are cited in \secref{sec:experiments}.
    \item The license information of the assets, if applicable. [Yes] All assets are open source (BoTorch, Gymnasium and Bayesmark under MIT or Apache-2.0 licenses, YAHPO Gym under Apache-2.0, UCI datasets through scikit-learn under BSD-3); no license restricts the use made here.
    \item New assets either in the supplemental material or as a URL, if applicable. [Yes] The implementation is released in the supplementary material.
    \item Information about consent from data providers/curators. [Not Applicable] Only public benchmark data are used.
    \item Discussion of sensible content if applicable, e.g., personally identifiable information or offensive content. [Not Applicable] The benchmarks contain no personal or offensive content.
  \end{enumerate}

  \item If you used crowdsourcing or conducted research with human subjects, check if you include:
  \begin{enumerate}
    \item The full text of instructions given to participants and screenshots. [Not Applicable] No human subjects.
    \item Descriptions of potential participant risks, with links to Institutional Review Board (IRB) approvals if applicable. [Not Applicable] No human subjects.
    \item The estimated hourly wage paid to participants and the total amount spent on participant compensation. [Not Applicable] No human subjects.
  \end{enumerate}

\end{enumerate}

